AgentCF: Collaborative Learning with Autonomous Language Agents for Recommender Systems

Recently, there has been an emergence of employing LLM-powered agents as believable human proxies, based on their remarkable decision-making capability. However, existing studies mainly focus on simulating human dialogue. Human non-verbal behaviors, such as item clicking in recommender systems, although implicitly exhibiting user preferences and could enhance the modeling of users, have not been deeply explored. The main reasons lie in the gap between language modeling and behavior modeling, as well as the incomprehension of LLMs about user-item relations. To address this issue, we propose AgentCF for simulating user-item interactions in recommender systems through agent-based collaborative filtering. We creatively consider not only users but also items as agents, and develop a collaborative learning approach that optimizes both kinds of agents together. Specifically, at each time step, we first prompt the user and item agents to interact autonomously. Then, based on the disparities between the agents' decisions and real-world interaction records, user and item agents are prompted to reflect on and adjust the misleading simulations collaboratively, thereby modeling their two-sided relations. The optimized agents can also propagate their preferences to other agents in subsequent interactions, implicitly capturing the collaborative filtering idea. Overall, the optimized agents exhibit diverse interaction behaviors within our framework, including user-item, user-user, item-item, and collective interactions. The results show that these agents can demonstrate personalized behaviors akin to those of real-world individuals, sparking the development of next-generation user behavior simulation.

==> preliminaries.tex <==
\section{PRELIMINARIES}


In this section, we introduce several key modules in the implementation of agent simulations.

\paratitle{Memory Module.}
During the process of interactions, agents tend to generate large amounts of experiences. 
However, given the limited context window size of LLMs, it becomes impractical to input all of this information for reasoning. Therefore, the inclusion of a memory module is imperative for building agents that can store a list of their experiences. In our work, we equip each user agent $u$ with both long-term memory $M_u^l$ and short-term memory $M_u^s$, which respectively capture their long-term and short-term preferences. Additionally, for each item agent $i$, we incorporate a unified memory module $M_i$ to record their global characteristics. When confronted with a new situation, the agent can retrieve relevant experience from its memory to provide informed responses.

\paratitle{Reflection Module.}
Compared to traditional methods that employ scalar gradients for model optimization, reflective agents leverage linguistic reflection to summarize their past failures and utilize them as "semantic" gradients to adjust relevant memory. This capability empowers agents to improve their decision-making processes in subsequent experiments. In this paper, we consider agents' inconsistent interactions with real users as failures, and thus we prompt the agents to reflect on the reasons accordingly. By doing so, the agents can optimize their memory toward the preferences and features of real-world individuals, thereby ultimately improving the simulation of interactions.

